Hyper-SD: Trajectory Segmented Consistency Model for Efficient Image Synthesis

Recently, a series of diffusion-aware distillation algorithms have emerged to alleviate the computational overhead associated with the multi-step inference process of Diffusion Models (DMs). Current distillation techniques often dichotomize into two distinct aspects: i) ODE Trajectory Preservation; and ii) ODE Trajectory Reformulation. However, these approaches suffer from severe performance degradation or domain shifts. To address these limitations, we propose Hyper-SD, a novel framework that synergistically amalgamates the advantages of ODE Trajectory Preservation and Reformulation, while maintaining near-lossless performance during step compression. Firstly, we introduce Trajectory Segmented Consistency Distillation to progressively perform consistent distillation within pre-defined time-step segments, which facilitates the preservation of the original ODE trajectory from a higher-order perspective. Secondly, we incorporate human feedback learning to boost the performance of the model in a low-step regime and mitigate the performance loss incurred by the distillation process. Thirdly, we integrate score distillation to further improve the low-step generation capability of the model and offer the first attempt to leverage a unified LoRA to support the inference process at all steps. Extensive experiments and user studies demonstrate that Hyper-SD achieves SOTA performance from 1 to 8 inference steps for both SDXL and SD1.5. For example, Hyper-SDXL surpasses SDXL-Lightning by +0.68 in CLIP Score and +0.51 in Aes Score in the 1-step inference.

==> tables/tcd_comp.tex <==
\begin{wraptable}{r}{0.45\linewidth}
    \centering
    \small
    % \vspace{-0.2cm}
    \caption{Quantitative results on unified LoRAs.}
    \setlength\tabcolsep{3pt} 
    \begin{tabular}{cccccc}
        \toprule[1pt]
        {\multirow{2}[-3]{*}{\textbf{Arch.}}} & 
        {\multirow{2}[-3]{*}{\textbf{Step}}} & {\makecell{\textbf{CLIP}\\\textbf{Score}}} & 
        {\makecell{\textbf{Aes}\\\textbf{Score}}} & 
        {\makecell{\textbf{Image}\\\textbf{Reward}}} & 
        {\makecell{\textbf{Pick}\\\textbf{Score}}} \\
        
        \midrule[1pt]

        {\multirow{4}{*}{\makecell{\textbf{SD15}\\512px}}} & 
        {8} & 
        {30.73} & 
        {5.47} & 
        {0.53} & 
        {0.224} \\

        & {4} & 
        {31.07} & 
        {5.55} & 
        {0.53} & 
        {0.224} \\

        & {2} & 
        {31.21} & 
        {5.93} & 
        {0.45} & 
        {0.222} \\

        & {1} & 
        {30.87} & 
        {5.79} & 
        {0.29} & 
        {0.215} \\

        \midrule[1pt]

        {\multirow{4}{*}{\makecell{\textbf{SDXL}\\1024px}}} & 
        {8} & 
        {32.54} & 
        {5.83} & 
        {1.14} & 
        {0.233} \\

        & {4} & 
        {32.51} & 
        {5.52} & 
        {1.15} & 
        {0.234} \\

        & {2} & 
        {32.59} & 
        {5.71} & 
        {1.15} & 
        {0.234} \\

        & {1} & 
        {32.59} & 
        {5.69} & 
        {1.06} & 
        {0.226} \\
        
        \bottomrule[1pt]
    \end{tabular}
    \vspace{-0.2cm}
    \label{tab:tcd_quantitative}
    
\end{wraptable}
